Conversion Prediction Using Multi-task Conditional Attention Networks to Support the Creation of Effective Ad Creative

Accurately predicting conversions in advertisements is generally a challenging task, because such conversions do not occur frequently. In this paper, we propose a new framework to support creating high-performing ad creatives, including the accurate prediction of ad creative text conversions before delivering to the consumer. The proposed framework includes three key ideas: multi-task learning, conditional attention, and attention highlighting. Multi-task learning is an idea for improving the prediction accuracy of conversion, which predicts clicks and conversions simultaneously, to solve the difficulty of data imbalance. Furthermore, conditional attention focuses attention of each ad creative with the consideration of its genre and target gender, thus improving conversion prediction accuracy. Attention highlighting visualizes important words and/or phrases based on conditional attention. We evaluated the proposed framework with actual delivery history data (14,000 creatives displayed more than a certain number of times from Gunosy Inc.), and confirmed that these ideas improve the prediction performance of conversions, and visualize noteworthy words according to the creatives' attributes.

==> 041_distribusion_campaign.tex <==
\begin{comment}
\begin{figure}[tb]
    \centering
    \subfloat[Campaign Distribution of each Genres.]{
        \includegraphics[clip, width=\linewidth]{images/genre_grouped_campaigns.eps}
        \label{fig:dist_of_campaigns_per_genre}
    } \\
    \subfloat[Creative Distribution each Genres.]{
        \includegraphics[clip, width=\linewidth]{images/genre_grouped_creatives.eps}
        \label{fig:dist_of_creatives_per_genre}
    } \\
    \caption{Some distributions in our dataset. M means man, and W means woman.}
    \label{fig:dists_per_genre}
\end{figure}
\end{comment}

\begin{comment}
Here, some distributions in the dataset used for training and evaluation are shown in \figref{fig:dists_per_genre}.
\figref{fig:dist_of_campaigns_per_genre} shows the number of campaigns with genre, and \figref{fig:dist_of_creatives_per_genre} shows the number of creatives with genre.
The number of campaign and creatives of health food for women is the largest, and second to this, cosmetic campaign and creatives for women is the largest.
\end{comment}

==> 041_result_map.tex <==
%%result 01
\begin{table*}[tb]
\centering
\caption{
    Comparison of mean average precision (MAP) in the proposed model.
    At the time of MAP calculation, the threshold was set to the number of conversions being 1 or more and 10 or more conversions.
    }
\label{tab:result_of_MAP}
\begin{tabular}{@{}clcccc@{}}
\toprule
\multicolumn{2}{c}{\multirow{3}{*}{Model}}                                                            & \multicolumn{4}{c}{Mean average precision (MAP) {[}\%{]}}                          \\ \cmidrule(lr){3-6} 
\multicolumn{2}{c}{}                                                                                  & \multicolumn{2}{c}{\#CV \textgreater 1} & \multicolumn{2}{c}{\#CV \textgreater 10} \\ \cmidrule(lr){3-4} \cmidrule(l){5-6}
\multicolumn{2}{c}{}                                                                                  & Single-task        & \textbf{Multi-task}         & Single-task         & \textbf{Multi-task}         \\ \cmidrule(r){1-2} \cmidrule(l){3-6}
\multicolumn{2}{c}{SVR}                                                                               & \multicolumn{2}{c}{34.69}               & \multicolumn{2}{c}{8.97}                 \\ \cmidrule(r){1-2} \cmidrule(l){3-6}
\multicolumn{2}{c}{MLP}                                                                               & 35.54              & 36.24              & 8.75                & 9.56               \\ \cmidrule(r){1-2} \cmidrule(l){3-6}
\multirow{3}{*}{GRU}                                                          & Vanilla               & 34.34              & 36.13              & 8.03                & 9.37               \\
                                                                              & Attention             & 35.71              & 36.15              & 9.37                & 9.65               \\
                                                                              & \textbf{Conditional attention} & \textbf{35.75}     & \textbf{36.63}     & \textbf{9.65}       & \textbf{10.05}     \\ \cmidrule(r){1-2} \cmidrule(l){3-6}
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Bi-directional\\ GRU\end{tabular}} & Vanilla               & 35.51              & 36.03              & 9.58                & 9.80               \\
                                                                              & Attention             & 35.51              & 36.19              & 9.66                & 10.05              \\
                                                                              & \textbf{Conditional attention} & \textbf{35.64}     & \textbf{36.89}     & \textbf{10.05}      & \textbf{11.09}     \\ \bottomrule
\end{tabular}
\end{table*}

==> 042_map_equation.tex <==
\begin{comment}
MAP is the average score of average precision (AP). 
The AP measured the performance of the evaluation results based on precision $p(\cdot)$ and recall $r(\cdot)$:
\begin{eqnarray}
    AP(u) = \sum_{k=1}^{N} p(k) \Delta r(k).
\end{eqnarray}
where $\Delta r(k)$ is the change in recall from items $k-1$ to $k$.
MAP is calculated from the average of scores for APs obtained in each creative evaluation.
\begin{eqnarray}
    MAP = \frac{1}{|Q_R|} \sum_{q \in Q_R}^{} AP(q)
\end{eqnarray}
\end{comment}

==> 042_ndcg_equation.tex <==
\begin{comment}
\begin{eqnarray}
    DCG = r_{1} + \sum_{i=2}^{N} \frac{r_i}{\log_{2}{i}}.
\end{eqnarray}
where $r_i$ is the result of graded relevance at the $i$-th position.
DCG varies depending on the size of the query and system, so when comparing performances, NDCG, which is the normalized version of DCG, is used.
To calculate NDCG, ideal NDCG ($IDCG$), which is the maximum value of DCG, is used.
\begin{eqnarray}
    NDCG = \frac{DCG}{IDCG}
\end{eqnarray}
\end{comment}
